Data-Driven Modeling and Verification of Perception-Based Autonomous Systems

This paper addresses the problem of data-driven modeling and verification of perception-based autonomous systems. We assume the perception model can be decomposed into a canonical model (obtained from first principles or a simulator) and a noise model that contains the measurement noise introduced by the real environment. We focus on two types of noise, benign and adversarial noise, and develop a data-driven model for each type using generative models and classifiers, respectively. We show that the trained models perform well according to a variety of evaluation metrics based on downstream tasks such as state estimation and control. Finally, we verify the safety of two systems with high-dimensional data-driven models, namely an image-based version of mountain car (a reinforcement learning benchmark) as well as the F1/10 car, which uses LiDAR measurements to navigate a racing track.

==> randomstuff.tex <==
% og version
\subsubsection{Model Training and Data Labeling}
To train the LiDAR noise model, we collected and labeled training data from the experiments carried out in \cite{ivanov20a} as follows: For each experimental LiDAR scan $\ell_i$ and corresponding estimated position $x_i$, we collected canonical LiDAR scans $g_c(x_i)$ from a simulator along the estimated position trajectory. These canonical scans concatenated with position $(g_c(x_i), x_i)$ make up the training input data for the classifier. All LiDAR data is also normalized between $[-0.5, 0.5]$, and position data is normalized between $[0,1]$.

To determine the binary labels $n_i$ for the classifier, we need to choose a threshold $t$ that determines if a given LiDAR ray should be classified as reflected or not. For this, we consider if each ray in a given real scan $\ell_i$ is sufficiently larger than the corresponding ray in our canonical scan $g_c(x_i)$. If it is above some threshold $t$, we label it 1, otherwise 0. This is formalized below.
\begin{align*}
    n_i^d = \left\{ \begin{array}{lll} 0 &&\text{if } \ell_i^d-g_c(x_i) < t \\
      1 &&\text{if } \ell_i^d-g_c(x_i) \geq t,\end{array} \right.
\end{align*}

To choose the optimal threshold the captures the adversarial noise, we choose $t$ so as to minimize the MSE between the $\ell_i$ and our noised data $g_n(x_i, g_c(x_i);t)$, defined element wise below.
%
\begin{align*}
    g_n(x_i, g_c(x_i);t)^d = \left\{ \begin{array}{lll} g_c(x_i)^d &&\text{if } \ell_i - g_c(x_i) < t \\
      0.5 &&\text{if } \ell_i - g_c(x_i) \geq t,\end{array} \right.
\end{align*}
%
Thus, we performed an sweep across potential threshold values and find a $t^*$ such that $ \sum_i ||\ell_i - g_n(x_i, g_c(x_i);t)||$ is minimal. We then use the $t^*$ to generate labels $n_i$ and from this have constructed our training set. The classifier is then trained using a class-weighted binary cross entropy loss to account for the under representation of adversarial examples in the training data. Namely, the loss function used scaled the loss on adversarial examples (class 1) by 4 relative to the non-adversarial (class 0) loss. Training results for different network sizes are shown in Figure \ref{fig:f11_model_training}. All models were trained for 1000 epochs with learning rate 0.01 and batch size 250, then for 29,000 more epochs with learning rate of 0.001 and batch size of 25,042. A weight decay parameter of 0.1 was used consistently. 

% The denoiser was trained using pairs of real and canonical scans from the process above without position as follows: $\mathcal{D}_D = \{(\ell_i, g_c(x_i)) \}$. For the purpose of the verification task in this case study, we trained a network with a single hidden layer of 100 neurons with binary cross entropy loss and a weight decay parameter of 1.


%succinct version 1
\subsubsection{Model Training}
For the generative canonical model $g_c(x)$, we use a neural net with 2 hidden layers of 50 and 100 neurons and train it using BCE loss and weight decay of 1 on pairs $(x, y(x)$ where x is position and $y(x)$ is 600 pixel canonical environment images generated from the simulator. While the simulator renders 400x600 RGB images, we downsample and grayscale all training images to minimize networks size for verification. For the contrast noise model, $g_{\text{cont}}$, we train a network a single hidden layer of 50 neurons with BCE loss and weight decay of 5 on pairs $((g_c(x), \alpha), y(x, \alpha))$, where $y(x,\alpha)$ is a contrasted simulator image using Python Image Library and contrast parameter $\alpha$. The contrasted image is then downsampled and grayscaled. Similarly, the blur noise model, $g_{\text{blur}}$, is a network with a single hidden layer of 50 neurons trained with BCE loss and weight decay 10 on pairs $((g_c(x), \delta), y(x, \delta))$ where $y(x,\delta)$ a normalized version of the image $0.5y(x-\delta) + y_k +0.5y(x+\delta)$. That is, a canonical image with a lighter overlay of left and right shifted images. Finally all training images were normalized [0,1] and inverted so black pixels have value 1, and white pixels have value 0. The image models used Tanh activations on hidden layers and Sigmoid activation on output layers so all images outputs are normalized [0,1]. \TW{Insert here: more details about training and qualitative evaluation of models can be found at ...}\TW{I guess this section really needs to be cut more to exclude all low level details.}


\begin{align}
    \label{eq:mc_system_model}
    \begin{split}
    x_{k+1}, v_{k+1} &= f(x_k, v_k, u_k)\\
    y_k &= g_{blur}(g_c(x_k), \delta_k)\\
    u_k &= c(p(y_k),v_k)
    \end{split}
\end{align}
We next outline the training procedure for these networks, provide analysis of the quality of the generative models, then show verification results for system with contrasted, blurred, and the composition of contrasted and blurred images.

In total, we train 4 networks in this case study. First, we train a robust position estimator $p: y \rightarrow x$ which infers the position given a (potentially noisy) image observation $y$. Next, we train a generative canonical image model $g_c: x \rightarrow y$, which maps the x position to a 600 pixel gray scale canonical image of the environment, and two noiser models $g_{cont}:(y, \alpha) \rightarrow y_{cont}$ and $g_{blur}:(y, \delta) \rightarrow y_{blur}$ which are trained to map canonical images and their noise parameters $\alpha, \delta$ to contrasted or blurred images, respectively. We additionally utilize a pre-trained and verified controller $c:(x,v)\rightarrow u$ which given position and velocity, outputs the thrust control action. The system model is given below for the case of the blurred observations:\TW{I wonder if I should include the models for all three systems, or instead leave this general.} \RI{We're already at 9 pages, so we probably don't have space for that. Will probably need to remove the following equation, too.}
To train the canonical model, we generated a 2000 element training set $\mathcal{D}_c = \{(x^i, y^i)\}$ in which the $x^i$ are equally spaced across the entire state space $[-1.2, 0.6]$ and the $y^i$ are the corresponding target images. The $y^i$ are generated by manually setting the state of the mountain car environment to position $x^i$, rendering the image as an 400x600x3 RGB array, resizing to a 20x30x3 image with a linear interpolation downsampling filter, then converting to a single channel gray scale image like the one shown in Figure \ref{fig:mc_canonical}. 

To train the noiser models, we created contrast and blur datasets $\mathcal{D}_{cont} = \{((y^i, \alpha^j), y_{cont}^{20i+j})\}$ and  $\mathcal{D}_{blur} = \{((y^i, \delta^j), y_{blur}^{20i+j})\}$ with 40000 examples each. For for each of the 2000 canonical images in the canonical data set, we created 20 noised target versions at various noise levels. For contrasted images, the canonical image was contrasted using Python Image Library's ImageEnhance tool image \cite{} for 20 contrast level with $\alpha \in [0.3, 2]$ where $\alpha = 0.3$ corresponds to a low contrast image as seen in Figure \ref{fig:mc_contrasted}, $\alpha =1$ returns the canonical image, and $\alpha =2$ is a high contrast image. The blurred training images were generated by rendering a central image $y$ and and left and right images $y_l$ and $y_r$. The left and right images were rendered $\delta \in [0, 0.3]$ position units on either side of the central image. Then the resulting blurred image was computed as first as a weighted sum, $\hat y_{blur} = 0.5y_l+y+0.5y_r$, then was normalized $y_{blur} = \hat y_{blur}/\max(\hat y_{blur})$. Figure \ref{fig:mc_blurred} shows a blur target with an intermediate noise level $\delta = 0.2$.

To train the robust position estimator, we used all 80000 noisy images from the contrast and blur data sets and their corresponding positions as targets. Note that we did not include the canonical set in training as the contrast and blur sets contain canonical images where the noise parameters are $\alpha=1$ and $
\delta=0$. Additionally, we augmented the training data with 100000 fully synthetic images generated by composing the canonical model, the contraster, then the blurrer for 1000 positions and 10 of each noise level. Additionally, we note here the last layer of the position estimator outputs a shifted an scaled version of Tanh such that the output range is bounded on $[-1.2, 0.6]$, the state bounds for position.

Before training, all image data was normalized between $[0,1]$ and inverted so black pixels correspond to 1, and white pixels correspond to 0. These data sets were then used to train fully connected neural networks with binary cross entropy loss. Tanh was used as the activation for hidden layers, and Sigmoid was used as activation on the output layer. A summary of the architectures and training parameters can be found in Table \ref{tab:mc_training}.
\begin{table}[t]
    \centering
    \begin{tabular}{|p{2.2cm}|c|c|c|c|c|}
    \hline
        Model Size & 3x100 & 4x100 & 5x100  &  6x100 & 6x200\\
        \hline
        Whole Scan         Accuracy[\%] & 61& 77 & 87 & 98 & 100 \\
        \hline
        Total Absolute Control Error & 3700 & 2312 & 1485 & 774 &  594 \\
        \hline
    \end{tabular}
    \centering
    \caption{F1/10 Noiser Model Training Results}\label{tab:f11_model_training}
    
\end{table}


\begin{table}[t]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \multicolumn{1}{c}{Network} & \multicolumn{1}{c}{\rot{Input Size}} &  \multicolumn{1}{c}{\rot{Layer Sizes}} &  \multicolumn{1}{c}{\rot{Output Size}}  &    \multicolumn{1}{c}{\rot{Output Activation}} &  \multicolumn{1}{c}{\rot{Weight Decay}} &  \multicolumn{1}{c}{\rot{Training Set}} \\
        \hline
        Canonical Generator $g_c$& 1 & 50, 100 & 600 & Sigmoid & 1 & $\mathcal{D}_c$ \\
        \hline
        Contraster $g_{cont}$ & 601 & 50 & 600 & Sigmoid & 5 & $\mathcal{D}_{cont}$ \\
        \hline
        Blurrer $g_{blur}$ & 601 & 10 & 600 & Sigmoid & 10 & $\mathcal{D}_{blur}$ \\
        \hline
        Position Estimator $p$ & 600 & 20, 20, 20 & 1 & Tanh &0.001 & $\mathcal{D}_{pos}$\\
        \hline
    \end{tabular}
    \caption{Network Architectures and training parameters for MC networks.}\label{tab:mc_training}
    
\end{table}

\subsubsection{Model Training and Data Labeling}
To train the LiDAR noise model, we collected and labeled training data from the experiments carried out in \cite{ivanov20a} as follows: For each experimental LiDAR scan $\ell_i$ and corresponding estimated position $x_i$, we collected canonical LiDAR scans $g_c(x_i)$ from a simulator along the estimated position trajectory. These canonical scans concatenated with position $(g_c(x_i), x_i)$ make up the training input data for the classifier. All LiDAR data is also normalized between $[-0.5, 0.5]$, and position data is normalized between $[0,1]$.

To determine the binary labels $n_i$ for the classifier, we need to choose a threshold $t$ that determines if a given LiDAR ray should be classified as reflected or not. For this, we consider if each ray in a given real scan $\ell_i$ is sufficiently larger than the corresponding ray in our canonical scan $g_c(x_i)$. If it is above some threshold $t$, we label it 1, otherwise 0. This is formalized below.
\begin{align*}
    n_i^d = \left\{ \begin{array}{lll} 0 &&\text{if } \ell_i^d-g_c(x_i) < t \\
      1 &&\text{if } \ell_i^d-g_c(x_i) \geq t,\end{array} \right.
\end{align*}

To choose the optimal threshold the captures the adversarial noise, we choose $t$ so as to minimize the MSE between the $\ell_i$ and our noised data $g_n(x_i, g_c(x_i);t)$, defined element wise below.
%
\begin{align*}
    g_n(x_i, g_c(x_i);t)^d = \left\{ \begin{array}{lll} g_c(x_i)^d &&\text{if } \ell_i - g_c(x_i) < t \\
      0.5 &&\text{if } \ell_i - g_c(x_i) \geq t,\end{array} \right.
\end{align*}
%
Thus, we performed an sweep across potential threshold values and find a $t^*$ such that $ \sum_i ||\ell_i - g_n(x_i, g_c(x_i);t)||$ is minimal. We then use the $t^*$ to generate labels $n_i$ and from this have constructed our training set. The classifier is then trained using a class-weighted binary cross entropy loss to account for the under representation of adversarial examples in the training data. Namely, the loss function used scaled the loss on adversarial examples (class 1) by 4 relative to the non-adversarial (class 0) loss. Training results for different network sizes are shown in Figure \ref{fig:f11_model_training}. All models were trained for 1000 epochs with learning rate 0.01 and batch size 250, then for 29,000 more epochs with learning rate of 0.001 and batch size of 25,042. A weight decay parameter of 0.1 was used consistently. 

The denoiser was trained using pairs of real and canonical scans from the process above without position as follows: $\mathcal{D}_D = \{(\ell_i, g_c(x_i)) \}$. For the purpose of the verification task in this case study, we trained a network with a single hidden layer of 100 neurons with binary cross entropy loss and a weight decay parameter of 1.
